Robust Communication Complexity of Matching: EDCS Achieves 5/6 Approximation

We study the robust communication complexity of maximum matching. Edges of an arbitrary $n$-vertex graph $G$ are randomly partitioned between Alice and Bob independently and uniformly. Alice has to send a single message to Bob such that Bob can find an (approximate) maximum matching of the whole graph $G$. We specifically study the best approximation ratio achievable via protocols where Alice communicates only $\widetilde{O}(n)$ bits to Bob. There has been a growing interest on the robust communication model due to its connections to the random-order streaming model. An algorithm of Assadi and Behnezhad [ICALP'21] implies a $(2/3+\epsilon_0 \sim .667)$-approximation for a small constant $0 < \epsilon_0 < 10^{-18}$, which remains the best-known approximation for general graphs. For bipartite graphs, Assadi and Behnezhad [Random'21] improved the approximation to .716 albeit with a computationally inefficient (i.e., exponential time) protocol. In this paper, we study a natural and efficient protocol implied by a random-order streaming algorithm of Bernstein [ICALP'20] which is based on edge-degree constrained subgraphs (EDCS) [Bernstein and Stein; ICALP'15]. The result of Bernstein immediately implies that this protocol achieves an (almost) $(2/3 \sim .666)$-approximation in the robust communication model. We present a new analysis, proving that it achieves a much better (almost) $(5/6 \sim .833)$-approximation. This significantly improves previous approximations both for general and bipartite graphs. We also prove that our analysis of Bernstein's protocol is tight.

==> temp.tex <==

By \cref{cl:large-matching,cl:glate-approximates-g},
we will assume in the remainder of this section that
$\mu(G) = \Omega(\log n \cdot \epsilon^{-2})$
and $\mu(E_r) \geq (1 - 2\epsilon)\mu(G)$.

\begin{claim} 
%[(Claim 2.1 in \cite{Bernstein20})]
\label{cl:large-matching}
    Without loss of generality, we can assume $\mu(G) = \Omega\paren{\log n \cdot \epsilon^{-2}}$.
\end{claim}
\begin{proof}
    A charging argument can be used to show that
    the number of edges in $G$ is less than $2 n \mu(G)$.
    Fix a maximum matching $M$ in $G$.
    For any edge $e$, 
    charge a unit to an edge of $M$ that is adjacent to $e$.
    Such an edge must exist since $M$ is a maximum matching.
    This way, we charge once for every edge in $G$,
    and every edge of $M$ is charged at most $n$ times
    through each of its endpoints.
    
    To see why the claim is true,
    note that in case $\mu(G)$ is too small,
    i.e.\ $\mu(G) = \O(\log n \cdot \epsilon^{-2})$,
    the number of edges in the graph will be $\O(n \log n \cdot \epsilon^{-2})$ and
    Alice can send the whole graph to Bob.
\end{proof}

\begin{claim} 
%[(Lemma 2.2 in \cite{Bernstein20})]
\label{cl:glate-approximates-g}
    Assuming $\mu(G) = \Omega\paren{\log n \cdot \epsilon^{-2}}$,
    it holds that $\mu(E_r) \geq (1 - 2\epsilon) \mu(G)$
    with high probability.
\end{claim}
\begin{proof}
    We use the \hyperref[chernoff]{Chernoff bound}.
    Fix a maximum matching $M$ in $G$.
    For every edge $e$ in $M$,
    let $X_e$ be a random variable that indicates if $e$ was not sampled in $E_s$.
    And let $X = \sum_{e \in M} X_e$.
    Then, it holds that $\expect{X_e} = 1 - \epsilon$,
    and $\expect{X} = (1 - \epsilon)\mu(G)$.
    By applying the Chernoff bound we get:
    \begin{equation*}
    \prob{\mu(E_r) \leq (1 - 2\epsilon) \mu(G)}
    \leq \prob{X \leq (1 - 2\epsilon) \mu(G)}
    \leq \exp\paren{-\Omega\paren{\epsilon^2 \mu(G)}}
    \leq \frac{1}{\poly(n)}. \qedhere    
    \end{equation*}
\end{proof}
